Predicting polaron mobility in organic semiconductors with the Feynman variational approach

We extend the Feynman variational method applied to the parabolic-band Fr\"ohlich (continuum) large polaron~\cite{Feynman1955} to a Holstein (lattice) small polaron, with a parabolic-band. This new theory shows a discrete localisation as a function of coupling strength. Having build the theory with the same quasi-particle Lagrangian as the 1955 work, we can directly use the FHIP~\cite{Feynman1962} response theory to calculate DC mobility and complex conductivity. We show that we can take matrix elements from electronic structure calculations on real materials, by modelling charge-carrier mobility in crystalline Rubrene. Good agreement is found to measurement, with a predicted mobility of $\mu = 47.72$~\si{cm^2 V^{-1} s^{-1}} at $300$~\si{K}.

==> results/Makefile <==
# Specify the path to the Julia executable
# JULIA_PATH := /Applications/Julia-1.8.app/Contents/Resources/julia/bin/julia
JULIA_PATH := /home/neutrino/julia-1.9.2/bin/julia
# JULIA_PATH := /opt/julia-1.9.2/bin/julia
# JULIA_PATH := /home/neutrino/julia-1.9.3/bin/julia

# Directories
DATA_DIR := data
PLOT_DIR := plots

NUM_THREADS ?= auto

# List of Julia scripts and corresponding CSV and plot files
JULIA_DATA_SCRIPTS := $(wildcard *data.jl)
JULIA_PLOT_SCRIPTS := $(wildcard *plot.jl)
DATA_FILES := $(patsubst %.jl, $(DATA_DIR)/%.jld, $(JULIA_DATA_SCRIPTS))
PLOT_FILES := $(patsubst %.jl, $(PLOT_DIR)/%, $(JULIA_PLOT_SCRIPTS))

# List of package dependencies
PKG_DEPS := Unitful

# Specific Holstein & K-Space commit 440
POLARON_URL := https://github.com/jarvist/PolaronMobility.jl
# POLARON_URL := ../../../Code/PolaronMobility.jl

# Rule to create directories if they don't exist
$(DATA_DIR) $(PLOT_DIR):
	mkdir -p $@

# Rule to create and activate Julia environment
define JULIA_ACTIVATE
	$(JULIA_PATH) -e 'using Pkg; Pkg.activate("env"); Pkg.instantiate(); $(foreach pkg,$(PKG_DEPS), Pkg.add("$(pkg)");); Pkg.add(url="$(POLARON_URL)", rev="holstein"); Pkg.precompile()'
endef

# Rule to run Julia scripts and generate CSV files
define JULIA_RUN
	@echo "Generating data: $@"
	$(JULIA_PATH) --project=env --threads $(NUM_THREADS) $<
endef

# Rule to generate plots from CSV files
define PLOT_RUN
	@echo "Generating plot: $@"
	TITLE=$$(grep -m 1 '^# Title:' $< | sed 's/^# Title: //'); \
	XLABEL=$$(grep -m 1 '^# X Label:' $< | sed 's/^# X Label: //'); \
	YLABEL=$$(grep -m 1 '^# Y Label:' $< | sed 's/^# Y Label: //'); \
	LEGEND=$$(grep -m 1 '^# Legend:' $< | sed 's/^# Legend: //'); \
	XLOG=$$(grep -m 1 '^# X Log:' $< | sed 's/^# X Log: //'); \
	YLOG=$$(grep -m 1 '^# Y Log:' $< | sed 's/^# Y Log: //'); \
	XRANGE=$$(grep -m 1 '^# X Range:' $< | sed 's/^# X Range: //'); \
	YRANGE=$$(grep -m 1 '^# Y Range:' $< | sed 's/^# Y Range: //'); \
	XTICS=$$(grep -m 1 '^# X Tics:' $< | sed 's/^# X Tics: //'); \
	YTICS=$$(grep -m 1 '^# Y Tics:' $< | sed 's/^# Y Tics: //'); \
	LINESTYLE=$$(grep -m 1 '^# Linestyle:' $< | sed 's/^# Linestyle: //'); \
	echo "Title: $$TITLE"; \
	echo "X Label: $$XLABEL"; \
	echo "Y Label: $$YLABEL"; \
	echo "Legend: $$LEGEND"; \
	echo "X Log: $$XLOG"; \
	echo "Y Log: $$YLOG"; \
	echo "X Range: $$XRANGE"; \
	echo "Y Range: $$YRANGE"; \
	echo "X Tics: $$XTICS"; \
	echo "Y Tics: $$YTICS"; \
	echo "Linestyle: $$LINESTYLE"; \
	echo "title='$$TITLE' ; xlabel='$$XLABEL' ; ylabel='$$YLABEL' ; xlog='$$XLOG' ; ylog='$$YLOG' ; legend='$$LEGEND' ; yrange='$$YRANGE' ; xrange='$$XRANGE' ; xtics = '$$XTICS' ; ytics = '$$YTICS' ; linestyle = '$$LINESTYLE' ; input_file='$<' ; output_file='$@'" | cat - plot.gnu | gnuplot
	echo "\n"
endef

# Main target to generate all data files
# all: $(DATA_FILES) $(PLOT_FILES) 

data: $(DATA_FILES)

plots: $(PLOT_FILES) 

# Clean rule to remove generated files
clean:
	rm -rf $(DATA_DIR) $(PLOT_DIR) env

activate:
	$(JULIA_ACTIVATE)

# Individual rules for data and plot generation
define DATA_RULE_TEMPLATE
$(DATA_DIR)/$(1).jld : $(1).jl | $(DATA_DIR)
	$$(JULIA_RUN)
endef

define PLOT_DATA_RULE_TEMPLATE
$(DATA_DIR)/$(1).data : $(1).jl | $(DATA_DIR)
	$$(JULIA_RUN)
endef

define PLOT_RULE_TEMPLATE
$(PLOT_DIR)/$(1) : $(DATA_DIR)/$(1).data | $(PLOT_DIR)
	$$(PLOT_RUN)
endef

$(foreach script,$(JULIA_DATA_SCRIPTS),$(eval $(call DATA_RULE_TEMPLATE,$(basename $(script)))))
$(foreach script,$(JULIA_PLOT_SCRIPTS),$(eval $(call PLOT_DATA_RULE_TEMPLATE,$(basename $(script)))))
$(foreach script,$(JULIA_PLOT_SCRIPTS),$(eval $(call PLOT_RULE_TEMPLATE,$(basename $(script)))))

# Specify the default target
.DEFAULT_GOAL := all

ifndef VERBOSE
.SILENT:
endif

.PHONY: deps activate clean

==> revision.tex <==
\newcommand{\Revision}{32539ae}

